EMMT: A simultaneous eye-tracking, 4-electrode EEG and audio corpus for multi-modal reading and translation scenarios

We present the Eyetracked Multi-Modal Translation (EMMT) corpus, a dataset containing monocular eye movement recordings, audio and 4-electrode electroencephalogram (EEG) data of 43 participants. The objective was to collect cognitive signals as responses of participants engaged in a number of language intensive tasks involving different text-image stimuli settings when translating from English to Czech. Each participant was exposed to 32 text-image stimuli pairs and asked to (1) read the English sentence, (2) translate it into Czech, (3) consult the image, (4) translate again, either updating or repeating the previous translation. The text stimuli consisted of 200 unique sentences with 616 unique words coupled with 200 unique images as the visual stimuli. The recordings were collected over a two week period and all the participants included in the study were Czech natives with strong English skills. Due to the nature of the tasks involved in the study and the relatively large number of participants involved, the corpus is well suited for research in Translation Process Studies, Cognitive Sciences among other disciplines.

==> Makefile <==
LATEX=pdflatex
MAINFILE=main

default: $(MAINFILE).pdf

$(MAINFILE).pdf: misc/sample.bib content.tex

%.pdf: %.tex
	$(LATEX) $<
	bibtex $* || ( echo "Bibtex failed" && exit 1 )
	# change the exit 1 to exit 0 in the line above if you want to ignore it
	lim=4; \
	  while [ $$lim -ge 0 ] \
	      && grep 'Rerun to get\|Citation.*undefined' $*.log >/dev/null 2>/dev/null; do \
	    $(LATEX) $< ; \
	    lim=$$(($$lim - 1)) ; \
	  done

.PHONY: ci
ci:
	# make sure git will remember my password
	git config credential.helper store
	# git pull push dance with possibly uncommited local modifications
	if git pull --no-edit; then echo No changes to hide; else git stash; git pull --no-edit; git stash apply; fi; git commit -am "make ci by $(USER)"; git push

clean:
	rm -f $(MAINFILE).log $(MAINFILE).aux $(MAINFILE).bbl $(MAINFILE).blg $(MAINFILE).toc $(MAINFILE).out $(MAINFILE).run.xml $(MAINFILE).bcf

